Very Weak Space-Time Variational Formulation for the Wave Equation: Analysis and Efficient Numerical Solution

We introduce a very weak space-time variational formulation for the wave equation, prove its well-posedness (even in the case of minimal regularity) and optimal inf-sup stability. Then, we introduce a tensor product-style space-time Petrov-Galerkin discretization with optimal discrete inf-sup stability, obtained by a non-standard definition of the trial space. As a consequence, the numerical approximation error is equal to the residual, which is particularly useful for a posteriori error estimation. For the arising {discrete linear systems} in space and time, we introduce efficient numerical solvers that appropriately exploit the equation structure, either at the preconditioning level or in the approximation phase by using a tailored Galerkin projection. This Galerkin method shows competitive behavior concerning {wall-clock} time, accuracy and memory as compared with a standard time-stepping method in particular in low regularity cases. Numerical experiments with a 3D (in space) wave equation illustrate our findings.

==> Data/3D-example2CG.tex <==


% Load the Data
\pgfplotstableread{Data/3DRadialExample2-CG-opt-exact-0-maxIt-1000-tolerance-1e-05-toleranceRes-0.01.txt}\ThreeDRadialTwoCGOptFalse
%\pgfplotstableread{Data/3DRadialExample2-CG-opt-exact-1-maxIt-1000-tolerance-0.0001-toleranceRes-0.1.txt}\ThreeDRadialTwoCGOptTrue
\pgfplotstableread{Data/3DRadialExample2-CG-lyap-exact-0-maxIt-1000-tolerance-1e-05-toleranceRes-0.01.txt}\ThreeDRadialTwoCGLyapFalse
%\pgfplotstableread{Data/3DRadialExample2-CG-lyap-exact-1-maxIt-1000-tolerance-0.0001-toleranceRes-0.1.txt}\ThreeDRadialTwoCGLyapTrue
\pgfplotstableread{Data/3DRadialExample2-Galerkin-0-maxIt-1000-tolerance-1e-05-toleranceRes-0.01.txt}\ThreeDRadialTwoGalerkin
\pgfplotstableread{Data/3DRadialExample2-TS--tolerance-1e-06.txt}\ThreeDRadialTwoTimestepping
\pgfplotstableread{Data/3Drefinements.txt}\ThreeDRadialTwoCG
\pgfplotstableread{Data/3Drefinements.txt}\ThreeDRadialTwoGT


% Concatinate the columns in the right order
%\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGOptTrue}{[index] 3}] {errorCGOPTexact} {\ThreeDRadialTwo}
%\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGOptTrue}{[index] 2}] {timeCGOPTexact} {\ThreeDRadialTwo}

\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGOptFalse}{[index] 3}] {errorCGOPTinexact} {\ThreeDRadialTwoCG}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGOptFalse}{[index] 2}] {timeCGOPTinexact} {\ThreeDRadialTwoCG}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGOptFalse}{[index] 1}] {iterCGOPTinexact} {\ThreeDRadialTwoCG}

%\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGLyapTrue}{[index] 3}] {errorCGLYAPexact} {\ThreeDRadialTwo}
%\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGLyapTrue}{[index] 2}] {timeCGLYAPexact} {\ThreeDRadialTwo}


\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGLyapFalse}{[index] 3}] {errorCGLYAPinexact} {\ThreeDRadialTwoCG}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGLyapFalse}{[index] 2}] {timeCGLYAPinexact} {\ThreeDRadialTwoCG}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoCGLyapFalse}{[index] 1}] {iterCGLYAPinexact} {\ThreeDRadialTwoCG}


\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoGalerkin}{[index] 3}] {errorGalerkin} {\ThreeDRadialTwoGT}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoGalerkin}{[index] 2}] {timeGalerkin} {\ThreeDRadialTwoGT}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoGalerkin}{[index] 1}] {iterGalerkin} {\ThreeDRadialTwoGT}

\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoTimestepping}{[index] 2}] {errorTimestepping} {\ThreeDRadialTwoGT}
\pgfplotstablecreatecol[copy column from table={\ThreeDRadialTwoTimestepping}{[index] 1}] {timeTimestepping} {\ThreeDRadialTwoGT}




\hspace{-1cm}

% Table with the CG Values
\pgfplotstabletypeset[
%Rename the columns
%columns/Refinements/.style={column name={Refinement}},
%columns/errorCGOPTexact/.style={column name={$L_2$ error}},
%columns/timeCGOPTexact/.style={column name={Time}},
columns/errorCGOPTinexact/.style={column name={$L_2$-error}, column type = {|r}, sci},
columns/timeCGOPTinexact/.style={column name={Wall time [s]}, column type = {|r}, sci},
columns/iterCGOPTinexact/.style={column name={Iter.}, column type = {|r}, fixed},
%columns/errorCGLYAPexact/.style={column name={$L_2$ error}},
%columns/timeCGLYAPexact/.style={column name={Time}},
columns/errorCGLYAPinexact/.style={column name={$L_2$-error}, column type = {|r}, sci},
columns/timeCGLYAPinexact/.style={column name={Wall time [s]}, column type = {|r}, sci},
columns/iterCGLYAPinexact/.style={column name={Iter.}, column type = {|r|}, fixed},
columns/Time/.style={column type = {|r}, fixed},
columns/Space/.style={column type = {|r}, fixed},
precision=2,
skip rows between index={0}{1},
% Head row		
every head row/.style={
	before row={
		\hline
		  \multicolumn{2}{|c|}{Unknowns} 
		 %& \multicolumn{2}{c|}{CG opt (exact)}
		 & \multicolumn{3}{c|}{CG ($\mathbb{K}_\delta^\mathsf{T}\mathbb{M}_\delta^{-1} \mathbb{K}_\delta$)}
		% & \multicolumn{2}{c|}{CG lyap (exact)}
		 & \multicolumn{3}{c|}{CG (Sylvester)} \\
	},
	after row=\hline,
},
column type/.add={|}{},
every last row/.style={after row=\hline},
]{\ThreeDRadialTwoCG}

